Capturing Dynamics of Time-Varying Data via Topology

One approach to understanding complex data is to study its shape through the lens of algebraic topology. While the early development of topological data analysis focused primarily on static data, in recent years, theoretical and applied studies have turned to data that varies in time. A time-varying collection of metric spaces as formed, for example, by a moving school of fish or flock of birds, can contain a vast amount of information. There is often a need to simplify or summarize the dynamic behavior. We provide an introduction to topological summaries of time-varying metric spaces including vineyards [19], crocker plots [56], and multiparameter rank functions [37]. We then introduce a new tool to summarize time-varying metric spaces: a crocker stack. Crocker stacks are convenient for visualization, amenable to machine learning, and satisfy a desirable continuity property which we prove. We demonstrate the utility of crocker stacks for a parameter identification task involving an influential model of biological aggregations [58]. Altogether, we aim to bring the broader applied mathematics community up-to-date on topological summaries of time-varying metric spaces.

==> Reviews-WithNotesAndCompletedTasksDeleted.tex <==


Overall, I am very interested in this definition of crocker stacks as I think they have the potential to be an incredibly useful analysis tool for time-varying data to fill the vacuum left behind by the mathematical frustrations of multiparameter persistence. The experiments are also very interesting since despite the lack of stability, the Euclidean distance is clearly doing well for separating out the data. I hope the authors continue to work in the directions started in Section 6 and 7, but I do not think that this portion of the work is ready for publication in this venue. However, I do think that the rest of the paper can be published largely as is.


==> Reviews.tex <==
Referee #1 (Remarks to the Author):


\section{Main Comments}

The topic of the paper is methods for comparison of time-varying metric spaces through the lens of topological data analysis (TDA). The authors survey existing methods and introduce an enrichment of some of their previous work, moving from so-called crocker plots to more sensitive signatures called crocker stacks. Crocker stacks are shown to have a certain stability property---this is desirable, because Lipschitz comparisons of topology-based metrics are an important theoretical selling point for TDA. Experiments are performed on recovering parameters of a well-known parametric model for collective motion; therein, the performance of crocker plots and crocker stacks is compared to a traditional physics-based method and a standard TDA-based method.

Overall, the paper is well-written and the topic that it considers is highly interesting to the TDA community. Some high-level comments are included below, with detailed minor comments given in the following section.

\begin{enumerate}
\item The main objects of interest are time-varying metric spaces, but this concept is never precisely defined. One can infer what is meant by context, but this causes some issues with understanding some of the results appearing later in the paper. These are described in more detail below.
\item The main novel contribution of the paper is the introduction of the crocker stack. Its usefulness is tested empirically and is justified by some theoretical observations. There are some issues with both of these perspectives:
\begin{enumerate}
\item The experiments don't seem to show that there is a definitive benefit to using the crocker stacks over crocker plots. Moreover, it would be nice to see comparisons to other vectorizations of persistent homology.
\item As the authors draw attention to in the paper, the stability result obtained for crocker stacks is not of the type which is useful in practice.
\end{enumerate}
\end{enumerate}



\section{Minor Comments}

\begin{enumerate}
\item Page 2, second paragraph. Typo: ``The hollw..."
\item Page 2, second paragraph. It would be more effective to create a figure illustrating this example and to move the description to the caption of the figure.
\item Page 3, first paragraph of 2.1. A technical point: the description of persistent homology (PH) starts off using a filtration of topological spaces as the basic object of study. Next the authors say: ``As an example, a sequence of Vietoris-Rips complexes...", but VR complexes are abstract simplicial complexes whose geometric realizations don't play a part in the PH computation. It should be clarified that PH doesn't actually require nested topological spaces in order to operate.
\item Page 3, second paragraph of 2.1. The same intuitive description of what the Betti numbers capture already appears on the previous page.
\item Page 4, The rank invariant. ``The collection of all natural numbers $\mathrm{rank}(V(i) \to V(j))$...": the authors could clarify that it is not just the set of such natural numbers, but rather the function $(i,j) \mapsto \mathrm{rank}(V(i) \to V(j))$ which gives the rank invariant.
\item Page 5, first line. For the notation $d_b(\mathrm{PH}(\mathrm{VR}(X)),\mathrm{PH}(\mathrm{VR}(Y)))$, should there be some explicit dependence on degree, e.g., $\mathrm{PH}_k(\mathrm{VR}(X))$? Instead, it would be okay to mention that such a dependency is implicit, but is suppressed from the notation.
\item Page 7, last paragraph. Typo: ``In the more theoretical..." should be ``In a more theoretical...".
\item Page 8, first pagraph of section 4. This is the first time that notation for a time varying metric space is introduced, $\mathbf{X} = \{X_t\}_{t \in [0,T]}$. It strikes me that (as far as I can see), this concept is never really precisely defined. By context, I take it to be the case that the authors are interested in the situation where time varying metric spaces are of the form $(X,d_t)$, where $X$ is a finite set and $d_t$ is a metric on $X$ for each time $t$. Is this correct? This needs to be clarified; if the metric spaces are not all defined over the same set, then one would need to consider point correspondences between the metric spaces at different times. If we don't restrict to finite metric spaces, then there are other questions that one could ask, even if there is a fixed set $X$; e.g., should the metrics at different times all induce the same topology on $X$?
\item Page 9, second-to-last paragraph. ``As an example, see Figure 8." It would be better to have a simpler example illustrating this concept which appears in the paper closer to this definition.
\item Page 13, Figure 8. This is not a good visualization of the crocker stack, in my opinion. It's fine as a schematic, but I think that the authors should also include several frames of the crocker stack so that the reader can actually see how the crocker plot changes when $\alpha$ varies. As presented, it's hard to parse what's going on here.
\item Page 15, Figures 9 and 10. Could we also see the distance matrices for the crocker stacks?
\item Page 17, Table 1. I think that it would improve readability of these results if the authors bolded the top scores in each column.
\item Page 18, paragraph beginning ``Generally speaking,...". I don't know that this sentence is characterizing the results shown in Table 1 very well. For experiment 1, crocker plots get higher scores than stacks; for experiment 2, crocker plots get a PCA score boost of 10\% over crocker stacks. I would say that the results are generally mixed.
\item Page 19, sentence beginning ``With a few exceptions,...". Similar to the last comment, this statement doesn't seem to reflect the reported results in Table 3. In each column there is at least one single $\alpha$ which classifies at a rate equal to or above the full crocker stack.
\item Page 20, section 5.3.3. Was there a reason that the authors used a supremum over $t$-values; i.e., used $d_b^\infty$ rather than, say, $d_b^2$? Since the crocker stacks are being compared with Euclidean distance, it seems reasonable to at least try $d_b^2$ to compare the stacked persistence diagrams. Also, the authors mention that the computational cost of bottleneck distance is an issue here---why not vectorize the PDs using, say, the persistence images technique previously developed by two of the authors? This seems to be a fair comparison with crocker stacks and wouldn't require much more work to try. This sort of approach is mentioned in the conclusion as a future direction, but it seems to fit perfectly well as a baseline for the experiment in this paper.
\item Page 21, Figure 13. The authors might want to clarify that $Z$ is $\mathbb{R}^2$ with Euclidean distance, since a space $Z$ doesn't appear in the figure anywhere.
\item Page 22, ``The Gromov-Hausdorff distance is a metric when restricted to the class of compact metric spaces". This is not exactly true: it's a metric on the quotient space under the equivalence relation of isometry.
\item Page 24, Figure 14. The caption says ``the interleaving distance is 1", but I believe that this should be the erosion distance.
\item Page 26, paragraph beginning ``We remark that this is only a pseudo-metric". Similar to a comment above, ``unless one restricts attention to only compact metric spaces" should be changed to ``unless one restricts attention to isometry classes of compact metric spaces".
\item Page 26, Lemma 7.4. The lemma works on ``totally-bounded time-varying metric spaces", and this has me confused about the definition of a time-varying metric space. For finite metric spaces with time parameter in a compact interval, this would always be the case. So, is it not the case that the authors are focusing on finite metric spaces? This goes back to my comment above regarding the lack of a precise definition of a time-varying metric space.
\item Page 26, Definition 7.2. The previous comment leads to another issue. If we are not restricting to finite metric spaces, why do we know that $d_\mathrm{GH}^p$ is well-defined? That is, how do we know that the function
\[
t \mapsto d_\mathrm{GH}(X_t,Y_t)^p
\]
is integrable? This seems to require some assumed regularity about how the metrics vary over time.
\item Page 27, second paragraph of 7.4. Typos in the notation $\mathrm{PH}(\mathrm{VR}(()X_t))$ and $\mathrm{PH}(\mathrm{VR}(()Y_t))$.
\item Will code for the experiments in the paper be made open source? This would increase the impact of the paper.
\end{enumerate}




Referee #2 (Remarks to the Author):

This paper presents the new construction of Crocker stacks, which are a time-varying generalization of Crocker plots introduced previously by a subset of the authors.

These constructions take as input time-varying metrics spaces, where we have a fixed set $X$ and the metric changes with respect to a parameter $t$ resulting in metric space $X_t$. Crocker plots are constructed by returning for each $(t,\epsilon)$, the Betti number $\beta(VR(X_t,\epsilon))$ for the Vietoris-Rips complex at distance parameter $\epsilon$. Crocker stacks add a third dimension to this construction by further involving a parameter $\alpha$, which essentially smooths out the Crocker plots. More generally, given a time-varying persistence module $V$, which is a collection of persistence modules for each $t$, $\{V_t\}$, a crocker stack is defined to be
$$
f_V(t,\epsilon,\alpha) = \rank( V_t(\epsilon - \alpha) \to V_t(\epsilon + \alpha)).
$$
Beyond the novelty of the definition, the authors give results analyzing some standard flocking models in Section 5, and present theoretical analysis results in Sections 6 and 7.

Overall, I think the definition is interesting and certainly warrants further study. Where I am having difficulties with this paper is the disconnect between the computational experiments in Section 5 and the theory built in Section 6/7, in particular because (as even noted by the authors), Section 5 utilizes standard Euclidean distance between the Crocker stacks as input to the ML algorithms; while Section 6 points out that the constructions are not stable under this metric, and instead present bounds related to values differing by $\delta$. For a SIAM review article, I might suggest extracting Sections 6 and 7 into its own separate paper for inclusion in a more specialized journal where more discussion can be had of these stability issues. Since the experiments and constructions are clearly doing well, I think the paper could easily merit publication with Section 6 removed, and would be of interest to a broad audience in SIAM.

With that said, let me focus a bit on Section 6 and 7 since I think these need a great deal of editing before the paper can be published. First, I do believe the work as presented as correct, so this is more about presentation and clarity.
- The entire example based around Question 6.5 feels very out of place. The question statement itself is difficult to parse (perhaps some set theory statement in addition would help with clarity). I wish you would go into more detail about the erosion distance, but again, this is why I think this whole direction deserves its own paper.
- Fig 15 Do you mean every edge weight to be 1? What is the difference between the dashed and solid edges? This figure doesn't seem to be particularly helpful for understanding.
- Because "stability" has such a strong connotation in the TDA community (in particular, as a 1-Lipshitz operation with respect to chosen metrics), calling Thm 7.6 feels like a massive letdown, if not a complete bait-and-switch.

Overall, I am very interested in this definition of crocker stacks as I think they have the potential to be an incredibly useful analysis tool for time-varying data to fill the vacuum left behind by the mathematical frustrations of multiparameter persistence. The experiments are also very interesting since despite the lack of stability, the Euclidean distance is clearly doing well for separating out the data. I hope the authors continue to work in the directions started in Section 6 and 7, but I do not think that this portion of the work is ready for publication in this venue. However, I do think that the rest of the paper can be published largely as is.


## Minor Issues
- (Pg 2) typo "hollw"
- (Pg 3) "persistence complex": This doesn't feel like standard vocabulary to me, I would probably have just called this data a filtration whether I'm explicitly using the inclusion maps or not.
- (Pg 4) "Points which remain throughout the entirety of the filtration _are said to_ last to infinity."
- (Pg 4, sec 2.4) There needs to be some mention of the issue with the diagonal earlier otherwise, this definition will confuse readers new to the subject.
- (Pg 5) The notation seems to be expanding exponentially, consider replacing PH(VR(X)) with something simpler like Dgm(X).
- Overall, the placement of figures seems off, there are a lot of times that there are forward references to figures that are many many pages away.
- (Fig 4) I think there is something wrong with this figure, likely caused by not being particularly careful about where bars land to match with the dashed lines. Also some details need to be checked, I think the red $\alpha$-persistence line should actually be at $2\alpha$ to align with the $\alpha$-smoothing as defined. Further, after $\alpha$ smoothing, the bars change length from the original, so carefully aligning bars with the dahsed lines will make this example more useful.
- (Fig 8) I wish this plot was drawn with several panels next to each other. I understand that the goal is to show the movie-ness of the structure, but now I can't actually see what changes from one time to the next. A cartoon-style drawing like this closer to the definition would be very useful, then the later figures could be drawn to see what's actually happening in the computation.
- (Fig 9) Can you add titles to teh figures to make it easier to read?
- (table 4) Perhaps add the (0.61) into it's own column to be clear that the computation doesn't involve homology.
- (Defn 7.2) Fix overflowing math.
- Lemma 7.4 Did you ever define totally-bounded in the context of time-varying metric spaces?
- Pg 27 Typo with extra () in PH(VR()X_t)
- Thm 7.6 You already defined the $f_X$ and $f_Y$ notation
- The sentence after Thm 7.6 about Cech complexes seems very out of place and needs some more justification in any case.
- The second paragraph of the Conclusion feels like it should be the introduction instead. 
